NumGPT: Improving Numeracy Ability of Generative Pre-trained Models

Existing generative pre-trained language models (e.g., GPT) focus on modeling the language structure and semantics of general texts. However, those models do not consider the numerical properties of numbers and cannot perform robustly on numerical reasoning tasks (e.g., math word problems and measurement estimation). In this paper, we propose NumGPT, a generative pre-trained model that explicitly models the numerical properties of numbers in texts. Specifically, it leverages a prototype-based numeral embedding to encode the mantissa of the number and an individual embedding to encode the exponent of the number. A numeral-aware loss function is designed to integrate numerals into the pre-training objective of NumGPT. We conduct extensive experiments on four different datasets to evaluate the numeracy ability of NumGPT. The experiment results show that NumGPT outperforms baseline models (e.g., GPT and GPT with DICE) on a range of numerical reasoning tasks such as measurement estimation, number comparison, math word problems, and magnitude classification. Ablation studies are also conducted to evaluate the impact of pre-training and model hyperparameters on the performance.

==> sections/5-discussion.tex <==
\section{Discussion}
% 1. We have gone through trial-and-error process and learned some important lessons from the design of NumGPT.
We have gone through trial-and-error process and learned some important lessons from the design of NumGPT.

==> sections/backup/1-introduction-backup-20210908-0906.tex <==
\section{Introduction}
Pre-trained models such as GPT~\cite{radford2018improving,radford2019language,brown2020language} and BERT~\cite{devlin2018bert,liu2019roberta,lan2019albert} have made remarkable achievements in natural language processing. Through fully utilizing a large-scale unlabeled corpus, they have successfully gained state-of-the-art results in various kinds of natural language understanding tasks, such as GLUE~\cite{wang2018glue} and SuperGLUE~\cite{wang2019superglue}. 
% Moreover, with the development of computational resources, it has become possible to train deep neural network models with a large parameter size such as GPT-3~\cite{brown2020language} and Switch transformer~\cite{fedus2021switch}. These models have achieved significantly better performances in different NLP tasks, including news generation, question answering and so on.
%\yong{Zhihua, pls further check it.}

% larger models can be trained, and GPT-3~\cite{brown2020language} or Switch transformer~\cite{fedus2021switch} impress the researchers in NLP and even in the AI field. 

% 1. GPT-3 is very great LMs. However, it has poor numeracy performance when encountering large numberes. 
%Large scale pretrained language models also have obtain inspiring results in other tasks. 
%GPT-3~\cite{brown2020language} has successful ability to model language and obtains inspiring results. 
%GPT-3~\cite{brown2020language} also demonstrates that it is also a few shot learners for addition task. However, a limitation is observed. As the numbers increase in the question, the performance of GPT-3 drops down seriously. 

\begin{figure}[htb]
\centering 
\includegraphics[width=0.48\textwidth]{figs/conf_egg_3.pdf}
\caption{The confidence for GPT answering the questions related to the weight of an egg. The fluctuated curve reflects that GPT does not capture the continuous property of numbers.} 
\label{Fig.gpt_conf}
\end{figure}

% Although those results in language understanding are inspiring, some researchers  have also found that there are limitations to such large pre-trained models. 

Despite their inspiring performance in natural language understanding, these pre-trained language models still cannot do consistently well with tasks involving numbers~\cite{thawani2021representing}.
%They cannot do well with tasks involving numbers, which can be interpreted as numeracy. 
For example, as shown in Fig.~\ref{Fig.gpt_conf}, the confidence for GPT answering the questions related to the weight of an egg tends to oscillate with the changes of answers. It exposes that GPT does not fully learn the continuous property of the numbers regarding certain context. 
% \zhc{For example, if the GPT model is trained to answer questions involving numbers, like "How many grams is an egg?",
% it often cannot correctly answer the question and the model behaviors will be strange.
% As shown in~\autoref{Fig.bert_logits},
% XXXXXX} \yong{Zhihua, please paraphrase this sentence.}
% i.e., not continuous in the logits give for the questions and answers pairs (from 0 to 304), as shown in~\autoref{Fig.bert_logits}. 
% \zhihua{Not a good example, may need to replace with GPT example.}
Some researchers~\cite{wallace2019nlp, thawani2021representing} regard it as \textit{numeracy ability}.
% Their research from other perspective also support the conclusions that
Their research has also confirmed that
the large pre-trained model still cannot handle numerical information very well. The lacking of numeracy ability hinders those models from performing well on tasks requiring numeracy~\cite{wallace2019nlp}, which is prevalent in real world problems. 

A line of work has proposed methods to improve the numeracy ability of the neural model. 
%In recent years, there are some research focusing on injecting the numeracy into the model. 
For example, \citet{geva2020injecting} improve the numeracy via generating more training data including numbers. \citet{zhang2020language} transform the number in the text into a scientific notation form. However, it does not guarantee that the models can learn numerical knowledge from the perspective of magnitude and mathematical notation. 
Other studies attempt to design a numeral embedding to improve the numeracy ability. They demonstrate that their designed embeddings can perform well in probing tasks on numeracy~\cite{jiang2019learning, sundararaman2020methods}.
% Embedding trained. -> Incorporate them into the model. 
However, none of them pre-trains their model with numeral embeddings on a large corpus in a self-supervised manner.  Therefore, we want to seek suitable numeral embeddings and incorporate them in pre-training large-scale language models.
% However, they don't investigate incorporating the numeral embedding into the pre-trained language models (e.g., GPT) to improve their numeracy ability. Therefore, we want to seek suitable numeral embeddings and incorporate them in the pre-training stage of models.


Inspired by previous work~\cite{jiang2019learning, sundararaman2020methods, zhang2020language},
% and scientific notation,
we propose NumGPT, a general autoregressive language model that uses a prototype-based embedding to encode the \textit{mantissa} (or \textit{significand}) of the number and separate embeddings to encode the \textit{exponent} of the number. We believe the inductive bias introduced by the numerical embedding will allow the model to present the precision and magnitude of numbers separately and generalize better on the numeric related tasks.  We also design a numeral-aware loss function which enables the model to generate numbers as well as regular text tokens. 
% we propose a numeral embedding based on the scientific notation. 
To evaluate the performance of NumGPT, we synthesize several classification tasks such as measurement estimation, number comparison, and simple arithmetic problems. We also conduct experiments on a real dataset which focuses on magnitude classification, called Numeracy-600K~\cite{chen2019numeracy} to evaluate the numeral predictive ability of our model.
%After obtaining promising results, We further jointly pretrain the GPT model with the numeral embedding on the wikipedia dataset, finetune on MultiNLI and evaluate it on EQUATE dataset. 
Experiments demonstrate that our methods outperform the baseline models including GPT and GPT with DICE~\citep{sundararaman2020methods}. We further evaluate the generated text of NumGPT on a subset of the math word problem dataset, showing that our methods can generate better numerals. Ablation studies on the effect of pre-training and model hyperparameters are conducted to test whether they have a large impact on the model performance.
% We further pre-train the GPT model with the numeral embedding on the Wikipedia dataset and observe whether it can further improve the performance.
% Experiments demonstrate that our methods outperform the baseline models including GPT model in those tasks.
%\yong{Zhihua, please check my side comments.}

Our contributions can be summarized as follows:

\begin{itemize}
  \item We propose a novel NumGPT model, which integrates the specifically designed numeral representations and loss function into the GPT model.
  \item We evaluate the numeracy ability of models on a series of synthetic and real-world tasks, and NumGPT achieves superior performance among them.
\end{itemize}



% 2. The training corpus is limited. We need extrapolation performance. 
%We observe that the training corpus for GPT-3 cannot infinitely cover all combination of numbers in the question and then it is hard for GPT-3 to memorize all cases for numbers. Therefore, we are seeking an approach to make GPT-3 train on limited training corpus while preserving strong calculation ability when encountering large numbers. % Such ability is so called extrapolation ability. We reframe this problem as we want to improve the GPT-3 extrapolation performance.

% 3. We want to simplify and narrow down the problem.
%However, directly improving GPT-3 model ability is costly and impractical. Therefore, we choose to reduce the parameters of GPT and adopt the implementation of minGPT~\footnote{https://github.com/karpathy/minGPT}. Following the idea of curriculum learning, we design several simplified tasks to encourage us to inject the numerical reasoning ability into the models. Such tasks are so called 
%probing task, number comparison, addition classification, multiplication classification. We also further conduct experiments on Numeracy-600K and reframe the original magnitude classification to fact check classification.


% 4. Inspired by NALU, we want to combine NALU and minGPT to improve extrapolation performance. 
% Meanwhile, another group of researchers have proposed Neural Arithmetic Logic Units (NALU)~\cite{trask2018neural} to improve the extrapolation performance of neural networks and demonstrate that it can well behave in the simple function learning task, learning to track time, MNIST counting and addition. Several researches
% ~\cite{madsen2020neural, schlor2020inalu, heim2020neural} are further conducted to improve the stability and ability of NALU. Inspired by their research, we are seeking possibility for combining NALU and minGPT to improve the models’ extrapolation ability. 


% 1. GPT recently demonstrated great performance in various tasks, including XXX, XXX, XXX. 
% GPT recently demonstrated great performance in various tasks, including XXX, XXX, XXX. 

% 2. However, the numeral understanding ability of GPT is weak. For example, XXX.
% However, the numeral understanding ability of GPT is weak. For example, XXX.

% 3. In this paper, we propose numeral embedding enhanced GPT to address this problem. Inspired by the recent studies, XXX. 
%In this paper, we propose numeral embedding enhanced GPT to address this problem. Inspired by the recent studies, XXX. 

% 4. Our contributions can be summarized as:
%Our contributions can be summarized as:
